Knowledge Graphs Evolution and Preservation -- A Technical Report from ISWS 2019

One of the grand challenges discussed during the Dagstuhl Seminar "Knowledge Graphs: New Directions for Knowledge Representation on the Semantic Web" and described in its report is that of a: "Public FAIR Knowledge Graph of Everything: We increasingly see the creation of knowledge graphs that capture information about the entirety of a class of entities. [...] This grand challenge extends this further by asking if we can create a knowledge graph of "everything" ranging from common sense concepts to location based entities. This knowledge graph should be "open to the public" in a FAIR manner democratizing this mass amount of knowledge." Although linked open data (LOD) is one knowledge graph, it is the closest realisation (and probably the only one) to a public FAIR Knowledge Graph (KG) of everything. Surely, LOD provides a unique testbed for experimenting and evaluating research hypotheses on open and FAIR KG. One of the most neglected FAIR issues about KGs is their ongoing evolution and long term preservation. We want to investigate this problem, that is to understand what preserving and supporting the evolution of KGs means and how these problems can be addressed. Clearly, the problem can be approached from different perspectives and may require the development of different approaches, including new theories, ontologies, metrics, strategies, procedures, etc. This document reports a collaborative effort performed by 9 teams of students, each guided by a senior researcher as their mentor, attending the International Semantic Web Research School (ISWS 2019). Each team provides a different perspective to the problem of knowledge graph evolution substantiated by a set of research questions as the main subject of their investigation. In addition, they provide their working definition for KG preservation and evolution.

==> tex/dragon/def.tex <==
With the help of your tutor, provide a definition for Knowledge Graph Evolution and Preservation that applies to the perspective that your team is taking for this problem. Probably, this will be one of the last things you will do...


==> tex/dragon/resources.tex <==
\textit{[1 page]}

%\noindent
%List here what datasets are you using and why.


==> tex/dragon/rq.tex <==
\noindent

%The research questions take from the main subject of the school, which is what preserving and supporting the evolution of a Knowledge Graph means. The following research questions have been proposed: In particular, we focus on the possibility to automatically capture evolution within KGs, and how to achieve that. 



==> tex/introduction.tex <==



%Data Validity
In computer science, data validation is the process of ensuring data have undergone data cleansing to ensure they have data quality, that is, that they are both correct and useful. 
To this end, usually so-called validation rules or constraints are applied to check for correctness, meaningfulness, as well as for data security.
%Linked Data
Linked Open Data are considered as interlinked, structured, and publicly available datasets encoded and accessible via W3C standard protocols. 
Fine grained access is enabled by utilizing IRIs (International Resource Identifiers) as universal address schema for each single data item.
Linked Open Data can be retrieved and manipulated via HTTP (Hypertext Transfer Protocol) using standard Web access (i.e. port 80).
Furthermore, Linked Open Data is encoded via RDF (Resource Description Framework) that structures data values in terms of simple triples (subject, property, object) thereby enabling the implementation of knowledge graphs by the interlinking of data items within a local repository, but also and in particular with external Linked Open Data sources.
To exploit the real potential of Linked Open Data, the SPARQL query language enables sophisticated federated queries among them.

%LOD potential errors
Linked Open Data is based on the idea to realize the large-scale implementation of a lightweight Semantic Web. 
Due to its simplistic design principles, it has been possible to easily transfer large existing data repositories into a RDF representation. Furthermore, Linked Open Data has been created via automated analysis of natural language texts or other unstructured data. 
Thereby giving way to the introduction of errors, insufficencies, inaccuracies, ambiguities, misjudgements, etc.
Moreover, Linked Open Data has also been created directly from user inputs enabling further potential error including different levels of trustworthiness, reliability, and accuracy.
The very same holds for the introduction of interlinkings among different Linked Open Datasets.

%Ontologies
The semantic backend of Linked Open Data is ensured via ontologies providing a formal, machine understandable definition of properties, classes, their relationship among each other including potential constraints, as well as axiomatic rules.
For Linked Open Data, those ontologies are often made available in terms of RDF vocabularies providing canonical terms to be used to name properties and classes.
The formal definition of the ontology based on description logics mostly remains hidden to the end user but is accessible for automated evaluation and validation.
Ontologies may be manually defined or also automatically created via knowledge mining techniques.
However, both possible approaches might again lead to logical or structural errors and other insufficiencies that prevent Linked Open Data to make use of its full potential.

%Linked Data Validity
The potential of Linked Open Data lies in its ability for large scale data integration accompanied by fully automated machine understanding.
Yet, this vision fails if data quality in terms of Linked Data Validity cannot be guaranteed.

This paper has the goal to shade light on different aspects of Linked Data Validity. It is a collection of nine differently focused contributions provided by students of the International Semantic Web Research Summer School (ISWS 2018) in Bertinoro, Italy.
Overall, five different approaches have been taken into account, which will be outlined in the subsequent Parts:

\begin{itemize}
    \item Part \ref{part1}: \textbf{Contextual Linked Data Validity}. First, the Natural Language Processing perspective is taken into account with a special emphasis on context derived from text (cf. Chapter \ref{sec:42s}), while subsequently contextual dimensions for assessing LOD validity are defined and implemented as  SPARQL templates  to assess existing Knowledge Graphs (cf. Chapter \ref{sec:ravenclaw}).
    \item Part \ref{part2}: \textbf{Data Quality Dimensions for Linked Data Validity}. Here, the different dimensions of data quality are taken into account to propose an approach for the general improvement of Linked Data validity (cf. Chapter \ref{sec:gryffinder}).
    \item Part \ref{part3}: \textbf{Embedding Based Approaches for Linked Data Validity.} First, a generalized framework for linked data validity based on knowledge graph embeddings is discussed (cf. Chapter \ref{sec:hobbits}), followed by its application to the important use case of validating LOD against Common Sense Knowledge (Chapter \ref{sec:deloreans}.
    \item Part \ref{part4}: \textbf{Logic-Based Approaches for Linked Data Validity.} Here, the application of description logics-based approaches to ensure linked data validity is described such as learning logical constraints (cf. Chapter \ref{sec:mordor}, and extending SHACL with restrictions (cf. Chapter \ref{sec:dragons}.
    \item Part \ref{part5}: \textbf{Distributed Approaches for Linked Data Validity.} For sake of efficiency the implementation of Linked Data Validity requires a distributed approach. First, a combination of BLockchains and Linked Data is introduced applied to the usecase of validating personal data (cf. Chapter \ref{sec:hufflepuff}. Furthermore, an approach to tackle Linked Data incompleteness is presented (cf. Chapter \ref{sec:jedis}.
\end{itemize}



%\begin{quotation}
%    \say{\textit{The Semantic Web isn't just about putting data on the web. It is about making links, so that a person or machine can explore the web of data.  With linked data, when you have some of it, you can find other, related, data.}}   - \textit{Tim Berners-Lee}[]
   
%\end{quotation}

%Linked Open Data (LOD) is the interlinked structured publicly available RDF data in the Web, identified via URI and accessible via HTTP. In other words, LOD is the collection of documents on the web and the connections between them. Linked Data(LD) was proposed as a set best practices for publishing data on the Web. The concept of Linked Data was first outlined by Tim Berners-Lee in July 2006. In a published W3C design article[], Lee outlined the following four principles of Linked Data:
%\begin{itemize}
%    \item Use URIs as names for things.
%    \item Use HTTP URIs so that people can look up those names.
%    \item When someone looks up a URI, provide useful information, using the standards (RDF, SPARQL).
%    \item Include links to other URIs, so that they can discover more things. 
%\end{itemize}

%Since the commencement of LOD, many initiatives have been taken to publish data which has given rise to LD cloud. %From the very beginning 
%As a result, the LD cloud has now exploded into billions of triples belonging to many different domains such as Government data, Bio-Medical data, Scholarly data etc.. Many times these data are generated automatically such as text mining, data mining etc. without any human interception which give rise to errors or other issues. One such example is that, the %production of 
%DBpedia is generated by automatically extracting information from the Wikipedia infoboxes. This leads to a whole new research direction on how to validate Linked Data for correctness or completeness etc. i.e., \emph{Linked Data Validity}.

%Linked open data encode global-scale knowledge potentially available to any artificial intelligence tool that may want to benefit from it as background knowledge for supporting their task. Regardless the specific task that such tools aim to address, the reuse of such knowledge may be challenging for diverse reasons: semantic heterogeneity, provenance, etc. As identified by Heath[], \say{Linked Data might be outdated, imprecise, or simply wrong}. Hence, there arouses the necessity to delve into linked data validity, that is to support the assessment of the validity of a linked data statement (or of a group of statements i.e. a sub-graph) from different perspectives. 

%The notion of validity can be related to two different perspectives: 
%\begin{enumerate}
%    \item Internal perspective
%    \item External perspective
%\end{enumerate}
%The internal perspective is built on data quality dimensions such as: \textit{accuracy, completeness, consistency, and novelty}. These dimensions involve, on the one side, the data itself (A-box statements) and, on the other side, the ontologies that describe data (T-Box statements). 
 
%The external perspective is driven by typical issues and contents related to a specific domain of the data, that in some cases could bring different results in terms of validity compared to the internal one. To better understand both perspectives, consider the following assertion: \\
%\centerline{\textit{ex:book ex:isWrittenIn 2054}}. 

%On the other hand, from an internal point of view, this assertion is not valid, because a book can be written in the past and not in the future. Nevertheless, if this assertion models a scenario related to a science fiction set in the future, this statement is probably valid. Our intuition is that both perspectives should be considered and evaluated to effectively establish LD validity.
%Furthermore, the internal perspective of LOD validity has been studied in the light of logical (in)validity, decentralized approach using Block chain as well as federated query answering approach. 

%As already mentioned, the external perspective refers to domain specific contents of the data. It has been analyzed from the perspective of Natural Language Processing, temporal contextualization, common sense knowledge as well detecting anomalies in the LOD graph coupled with different approaches to tackle the issue. 

%From the external perspective, exemplary use cases for LOD validity have been studied as well as  validity metrics have been established that are sensible both/either to structure (internal), as well as to tasks, existing knowledge and sustainability (external). In another study, logical LOD validity has been studied in the light of logical techniques as well as logical techniques are explored there to regain logical LOD validity once it is lost. Also, different degrees of logical LOD (in)validity has been investigated. In another perspective, it was focused on how federated SPARQL query processing can be used to validate RDF data completeness and links between Linked Datasets. However, the data in the Web is overly massively centralized. Hence, it has also been studied on how Blockchains can provide a mechanism for this as a decentralised platform.


%Following these lines this report classifies the methodologies for Linked Data Validity into (i) external, (ii) internal perspectives. 


==> tex/jedi/readme.tex <==
all sections are in tex/jedi.tex

==> tex/klingon/resources.tex <==
\textit{[1 page]}

\noindent
List here what datasets are you using and why.

==> tex/ravenclaw/resources.tex <==
\textit{[1 page]}

\noindent
List here what datasets are you using and why.

==> tex/slytherin/02-def.tex <==




%With the help of your tutor, provide a definition for knowledge graph evolution and preservation that applies to the perspective that your team is taking for this problem. Probably, this will be one of the last things you will do...




==> tex/slytherin/05-resources.tex <==
%\textit{[1 page]}

%\noindent
%List here what datasets are you using and why.

==> tex/slytherin/07-evaluation.tex <==
\textit{[2 pages]}

\noindent
Show here that your proposed approach addresses your research questions or how you intend to show it. This can be done by either or both:

\begin{itemize}
    \item Describing an experimental setting design, including research hypotheses, methods and metrics of measurements 

    \item Describing a proof of concept/use case, based on real data, that support your claim
\end{itemize}



==> tex/vulcanian/rq.tex <==
Open Data has gained a lot of popularity and support by governments in terms of improving transparency and enabling new business models: Governments and public institutions, but also private companies, provide open access to raw data with the goal to present accountable records \cite{attard2015systematic}. Interlinking these Open Data is important in order to enrich it, make it more searcheable, and thereby contributes to the idea of a global knowledge graphs. This paper focuses on capturing the evolution of the knowledge graph, the datasets and the metadata by considering the following research questions:
\begin{itemize}
    \item \textbf{RQ1:} \textit{How can publishing organizations of open data knowledge sources be linked to existing knowledge graphs? Are the open data publishing organizations represented in knowledge graphs?} 
    % -> Vulcan Linker (sec 6.1)
    \item \textbf{RQ2:} \textit{How should mappings look like in order to account for knowledge graph evolution as well as evolution of the dataset (including the corresponding metadata)?}
    \item \textbf{RQ3:} \textit{How can organizational evolution be represented in a knowledge graph?}
    %\item \textbf{RQ3:} \textit{What are strategies that can be applied in order to detect which are the institutions who are publishing the datasets?}
    %\item \textit{How can knowledge graph and dataset evolution be considered in this linking process?}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%   THIS IS COMMENTED
\iffalse
JUST FOR REFERENCE, DELETE LATER: 

There arethe the initial questions proposed in Axel's presentset ation.

\begin{itemize}
    \item How can we align large evolving corpora of publicly available structure knowledge sources (Open Data Portals e.g. EU Open Data Portal) to Open KG (e.g. DBpedia, Wikidata, WorNet(s), BabelNet) and the Datasets in slides below?
    \item Can current models used by open knowledge graphs to integrate these sources and capture their evolution and context (e.g. Publishers, was previously, date of the modification, etc)?
    \item How can this metadata be completed? How can this metadata be aligned and linked? 
    \item How can we query data alongside with it’s contextual metadata?
    \item As starting point, we can use evolving (weekly crawled) corpus of Open Data portals’ metadata from 260 Open Data Portals.
    
    \item What are the strategies that should be applied in order to detect which are the institutions who are publishing the datasets.
\end{itemize}

Other questions after 03/07 Stand up:
\begin{itemize}
    \item What are the strategies that should be applied in order to detect which are the institutions who are publishing open datasets? ... using metadata as contact email, institution label, etc.
    \item Is there any way to track the differences between open datasets published by an institution before and after an election period?
\end{itemize}

\fi
%%%%%%%%%%%%%%%%%%%%   END OF COMMENT
